Smooth Boolean functions are easy: efficient algorithms for low-sensitivity functions

A natural measure of smoothness of a Boolean function is its sensitivity (the largest number of Hamming neighbors of a point which differ from it in function value). The structure of smooth or equivalently low-sensitivity functions is still a mystery. A well-known conjecture states that every such Boolean function can be computed by a shallow decision tree. While this conjecture implies that smooth functions are easy to compute in the simplest computational model, to date no non-trivial upper bounds were known for such functions in any computational model, including unrestricted Boolean circuits. Even a bound on the description length of such functions better than the trivial $2^n$ does not seem to have been known. In this work, we establish the first computational upper bounds on smooth Boolean functions: 1) We show that every sensitivity s function is uniquely specified by its values on a Hamming ball of radius 2s. We use this to show that such functions can be computed by circuits of size $n^{O(s)}$. 2) We show that sensitivity s functions satisfy a strong pointwise noise-stability guarantee for random noise of rate O(1/s). We use this to show that these functions have formulas of depth O(s log n). 3) We show that sensitivity s functions can be (locally) self-corrected from worst-case noise of rate $\exp(-O(s))$. All our results are simple, and follow rather directly from (variants of) the basic fact that that the function value at few points in small neighborhoods of a given point determine its function value via a majority vote. Our results confirm various consequences of the conjecture. They may be viewed as providing a new form of evidence towards its validity, as well as new directions towards attacking it.

==> content/learning.tex <==
% !TEX root =  sens-exact.tex






\subsection{Exact learning from uniform random examples}

\begin{Thm} \label{thm:learn}
There is an algorithm $L$ with the following property:  $L$ is given as input $s \geq 1$, $\delta > 0$ and access to i.i.d random examples $(x,f(x))$ where $f$ is an unknown function in ${\cal F}(s,n).$  $L$ draws $M(n,s,\delta)=2^{\poly(s,\log n, \log {\frac 1 \delta})}$ random examples and runs
in time $T(n,s,\delta) = 2^{\poly(s,\log n, \log {\frac 1 \delta})}$.
With probability $1-\delta$ outputs a Boolean formula $F$ of depth $O(s \log n)$ and size $n^{O(s)}$ such that $F(x)=f(x)
$ for all $x \in \{0,1\}^n.$
\end{Thm}

\begin{proof}
We recall the following Fourier concentration bound for sensitivity-$s$ functions:

\begin{Thm} \label{thm:FC}
If $f: \{0,1\}^n \to \{-1,1\}$ has $s(f) \leq s$, then we have
\begin{equation} \label{eq:FC}
\sum_{S \subseteq [n], |S| \geq O(s(\log 1/\eps)^{8})} \widehat{f}(S)^2 \leq \eps.
\end{equation}
\end{Thm}
We take $\eps = \delta / (3 {n \choose \leq 2s}),$
$m = {n \choose \leq C s \log(1/\eps)^8}$ for an absolute constant $C$, and $\tau = \eps.$  With these
parameters, the LMN algorithm works by drawing $M(n,s,\delta) = O({\frac m \tau} \log {\frac m \delta})$
uniform random examples $(x,f(x))$ and using them to obtain an estimate $c_S$ of  $\widehat{f}(S)$
for each $S \subseteq [n], |S| \leq  O(s(\log 1/\eps)^{8}).$  Its output hypothesis is $h: \{0,1\}^n \to \{-1,1\},$
\[
h(x) = \text{sign}\left(\sum_{S \subseteq [n], |S| \leq  O(s(\log 1/\eps)^{8})} c_S \chi_S(x) \right)
\]
where $\chi_S(x)$ is the parity function over the variables in $S$.  The Fourier concentration bound (\ref{eq:FC})
together with the performance guarantee of the LMN algorithm give that with probability
$1-\delta/3$, the hypothesis $h$ satisfies $\Pr_{x \in \{-1,1\}^n}[h(x) \neq f(x)] \leq \eps = \delta / (3 {n \choose \leq 2s}).$
A union bound over the ${n \choose \leq 2s}$ points in ${\cal B}(-1^n,s)$ gives that  $h(x)=f(x)$ for all 
$x \in {\cal B}(-1^n,s)$, with overall probability at least $1-2\delta/3$.  The hypothesis that the learning algorithm
outputs is the formula whose existence is established by Corollary \ref{cor:formula} (the remaining $\delta/3$ failure probability goes to the failure probability that the random coin tosses hard-wired into the formula construction
do not result in a formula correctly computing $f$).  \end{proof}


